METER: A Dynamic Concept Adaptation Framework for Online Anomaly Detection

Real-time analytics and decision-making require online anomaly detection (OAD) to handle drifts in data streams efficiently and effectively. Unfortunately, existing approaches are often constrained by their limited detection capacity and slow adaptation to evolving data streams, inhibiting their efficacy and efficiency in handling concept drift, which is a major challenge in evolving data streams. In this paper, we introduce METER, a novel dynamic concept adaptation framework that introduces a new paradigm for OAD. METER addresses concept drift by first training a base detection model on historical data to capture recurring central concepts, and then learning to dynamically adapt to new concepts in data streams upon detecting concept drift. Particularly, METER employs a novel dynamic concept adaptation technique that leverages a hypernetwork to dynamically generate the parameter shift of the base detection model, providing a more effective and efficient solution than conventional retraining or fine-tuning approaches. Further, METER incorporates a lightweight drift detection controller, underpinned by evidential deep learning, to support robust and interpretable concept drift detection. We conduct an extensive experimental evaluation, and the results show that METER significantly outperforms existing OAD approaches in various application scenarios.

==> secs/0.response.tex <==
\centerline{\textbf{\Large Response to Reviewers' Comments}}
\vspace{10mm}

\begin{multicols}{2}
% \setcounter{page}{1}
\pagestyle{empty}


\noindent 
To the Meta-Reviewer and Reviewers:

{
We would like to thank the meta-reviewer and reviewers for their valuable and constructive feedback on our manuscript.
We have carefully addressed each comment and concern raised by the reviewers and highlighted major changes in \textcolor{blue}{blue} font in the revised manuscript.
In this cover letter, we first summarize the major changes that we have made and then provide detailed responses to each reviewer's concerns.
}

\subsection*{Summary of Major Changes}
\begin{itemize}[leftmargin=*]
    %reviewer 1
    \item We have expanded the sensitivity study in Section~\ref{sec:exp_sensitivity} to elucidate the effects of the proportion of the historical data stream and the sliding window length.
    %%ooibc: what?
    \item We have added Section~\ref{sec:exp_efficiency} to provide an in-depth analysis of the efficiency of \name during both training and inference.
    \item We have more formally defined the online anomaly detection and concept drift problem in Section~\ref{sec:preliminary}.
    \item We have enhanced the analysis of the experimental results in Section~\ref{sec:exp_effectiveness}, Section~\ref{sec:exp_concept_drift}, and Section~\ref{sec:exp_ablation}. %(temporal dependencies, concept uncertainty in fig4, a well-trained vanilla autoencoder)
    \item We have improved and reorganized the related work in Section~\ref{sec:related work} to provide a more comprehensive review of relevant research in the field.
    %reviewer 2
    \item We have updated Section~\ref{sec:implementation_details} to provide more detailed descriptions of \name's settings and configurations, particularly parameter settings and hardware configurations. 
    %reviewer 3
    \item We have added a new challenging anomaly detection dataset as described in Section~\ref{sec:dataset} and reported new experimental results in Section~\ref{sec:exp_effectiveness}. 
    %\item We have updated Section~\ref{sec:introduction} to improve the presentation. (the novelty and contribution of the design of hypernetwork...)
    % experimental results to prove the observation that ‘static historical data typically encompass the majority of anomaly patterns and thus comprises the recurring central concepts’.
    \item We have extended Section~\ref{sec:exp_ablation} to test the flexibility of \name.
    \item We have improved the discussions of interpretability in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability}.
    \item To make space for the above changes, we 
    %have shortened Sections \ref{sec:preliminaries} and  \ref{sec:related-work}, and 
    have removed the following: the training pseudocode (i.e., the previous Algorithm~1), the dataset statistics table (i.e., the previous Table~1), the receiver operating characteristic curves of the top six methods on four real-world datasets (i.e., the previous Figure~3), the experimental results of the synthetic datasets and the corresponding performance analysis section (i.e., the previous Table~5 and Section~\ref{sec:exp_effectiveness}). We instead refer the readers to our online technical report\footnote{\label{note:tech_report}\url{https://drive.google.com/file/d/1ir2x4vL7r_RC3eaXlCZyVbzRVDpQua9L/view?usp=sharing}} for these results and analysis.
    %% jq: will update the url later on
\end{itemize}

\subsection*{Response to Meta-review}
\textbf{Comment 1:} The motivation, technical depth, and contribution of this paper needs to be made more clear. Some requires clarification, and some might potentially require new experiments.


\vspace{2mm}
\noindent
\textbf{Response.} 
%Thank you for your valuable comment. 
%We thank the meta-reviewer for your valuable feedback.
% In response to these valuable suggestions, w
Based on the suggestions, we have made substantial enhancements to our paper in terms of presentation, structure, and experimentation.

First, we have improved the Introduction, Preliminaries, and Related Work sections in the revised manuscript to offer a clearer presentation of the motivation, technical depth, and contributions.
Additionally, we have restructured the manuscript to improve the overall organization and coherence.

Second, we have also enhanced our experimental evaluations.
This includes an in-depth sensitivity analysis investigating the impact of key parameters, a series of new ablation studies to demonstrate the flexibility of our approach, and supplementary experiments that support the motivation and claims.
Further, we have added efficiency experiments and incorporated more challenging datasets into our evaluation as suggested.
%We also supplemented more detailed experimental configurations and discussion. 
Our experiments now comprise 17 real-world datasets and 15 baseline methods in total.

% We refer the reader to our online technical report\textsuperscript{\ref{note:tech_report}} for extensions to the other algorithms (including the training part of the enhanced protocol, and the model prediction parts of both protocols).

% All the comments have been carefully addressed, which significantly improves the quality of our manuscript.
% % We believe that the reviewer’s comments significantly improve the quality of our manuscript.
% The details of the revision are articulated in the subsequent responses.


\vspace{2mm}
\noindent
\textbf{Comment 2:} There are many clarifications that need to be made in the revised version.

% We thank you for your valuable feedback. 
\vspace{2mm}
\noindent
\textbf{Response.} In the revised manuscript, we have made clarifications accordingly to enhance the overall quality and clarity of our work.

These clarifications include formal definitions of the problem under investigation, more detailed experimental configurations, and an enhanced discussion section that provides deeper insights.
Also, we have expanded our analysis of interpretability and introduced new experiments to support our claims.

% Throughout this revision process, we have strived to ensure that every comment and suggestion from the reviewer has been thoughtfully considered and appropriately incorporated into the revised version. We believe that these efforts have significantly improved the overall quality of our manuscript, making it more accessible and informative.

All the comments from the reviewers have been carefully addressed,
%as suggested by respective reviewers, 
which has helped to significantly improve the quality of our manuscript.
% We believe that the reviewer’s comments significantly improve the quality of our manuscript.
The details of the revision made in response to reviewers' comments are articulated in the subsequent responses.

% formal definition, experiment， interpretability 


\subsection*{Response to Reviewer 1}
\textbf{D1:} (1) By pre-training an autoencoder on the historical data stream, the SCD module in METER attempts to learn the central concepts in data stream (as in Sec 3.2). Since the learned central concepts play a critical role in determining whether new concepts are coming, the proportion of the trained historical data stream could be an important parameter. However, there is no discussion of this parameter in either the model elaboration or sensitivity study phase. Intuitively, an insufficient amount of historical data stream can lead to a failure to learn sufficiently informative central concepts.

\vspace{2mm}
\noindent
\textbf{Response.}
%We thank you for your constructive feedback.
We have added more discussions and sensitivity studies to demonstrate the impact of the proportion of the trained historical data stream.
%%% ooibc: this
%%% what is this???

First, we have elaborated on the descriptions of the proportion of the historical data stream that is used to train \name in Section~\ref{sec:implementation_details}, which facilitates understanding of this important parameter.
Second, we have extended the sensitivity study in Section~\ref{sec:exp_sensitivity} to examine the effect of the proportion of the historical data stream $h_r$.
One important observation is that when $h_r$ is too small, the performance notably declines due to a lack of historical data in training, which results in a failure to acquire adequate information for learning central concepts.
As the ratio increases, there is a noticeable improvement in performance.
However, we find that a higher ratio does not guarantee better performance, suggesting that the model overfits the training data.
% , ultimately causing a reduction in performance during inference.
In contrast, the proposed OUS is more efficient and performs better than training models directly on more data.
The new results reveal that a historical data ratio of 0.2 can consistently achieve favorable results across datasets.
Therefore, we have set the value of $h_r$ to 0.2 in all experiments.


\vspace{2mm}
\noindent
\textbf{D1:} (2) In the experiments, the sliding window length of the offline updating strategy has been set to 64 by default for all datasets (as in Sec 4.1.4). Discussion and sensitivity study of this important parameter is expected. The window length parameter seems to determine how often the framework will be updated, which consequently decides both the training and inferring efficiency of the model.

\vspace{2mm}
\noindent
\textbf{Response.} %We thank you for this insightful advice.
%This parameter is indeed critical to OUS.
We have added discussions and extended the sensitivity study in Section~\ref{sec:exp_sensitivity} to provide a more thorough examination of \name's behavior under different sliding window lengths $\Delta L$.

We report the impact of the window size on both performance and efficiency in Table~\ref{tab:sentitive}.
Results show that a small $\Delta L$ results in frequent model updates, which can achieve better AUCROC performance while at the cost of longer inference time.
In contrast, a large $\Delta L$ reduces inference time but compromises the model capacity to capture concept changes timely, leading to noticeable performance degradation.
Fortunately, as discussed in Section~\ref{sec:exp_efficiency} the update time of the model is minimal, and the model exhibits good performance across a wide range of $\Delta L$, which allows users to adjust the window size to meet specific needs in various practical applications.

\vspace{2mm}
\noindent
\textbf{D1:} (3) Does the offline updating strategy (OUS) need to re-train the entire framework each time the accumulated concept uncertainty exceeds a given threshold? If so, how can the model be guaranteed to be efficient? Does the pre-defined threshold need to be updated? Although the paper states that a parallel training strategy is used, it lacks a detailed description.

\vspace{2mm}
\noindent
\textbf{Response.}
%\textcolor{red}{First, }
%%% ooibc: where is Second?
Regarding the offline updating strategy (OUS) and its impact on efficiency, OUS only fine-tunes the key modules instead of re-training the entire framework.
Specifically, OUS continuously monitors the concept uncertainty accumulated within a sliding window, and the accumulated concept uncertainty surpassing a predefined threshold indicates that the trained SCD, IEC, and DSD modules can no longer effectively handle the current data stream.
Therefore, the increased concept drift in the recent data streams requires an update of these key modules of the framework, ensuring that they adapt dynamically to the evolving data stream.
We have added more detailed descriptions of OUS in Section~\ref{sec:ous}.

% sf: will double check the word choice - negligible
In terms of efficiency, as demonstrated in the new results and discussions we have added in Section~\ref{sec:exp_ablation} and Section~\ref{sec:exp_efficiency}, the update time for the model is negligible, and the throughput is extremely high.
Further, one can control the update frequency of OUS by adjusting the window size $\Delta L$, thereby striking a trade-off between effectiveness and efficiency according to specific needs.

As for the threshold $\mu_{e}$, it is initially set to the largest value of concept uncertainty observed during training, and is updated automatically based on the incoming data stream.
Specifically, we adopt the exponential moving average (EMA) strategy~\cite{klinker2011exponential} to dynamically update this threshold during the offline updating process, which adapts to changing conditions as the model continues to learn from incoming data within the current sliding window.

Also, we have introduced a detailed description of the parallel training strategy in Section~\ref{sec:ous}.
Specifically, the parallel training strategy performs online OAD inference using the latest fine-tuned modules and meanwhile, fine-tunes key modules offline.
This decouples the training and inference for efficiency and modularity, and allows for executing OUS without affecting the online OAD inference service.

% We thank you for your insightful comments.
We have made clarifications and detailed descriptions accordingly in Section~\ref{sec:ous}, Section~\ref{sec:exp_ablation} and Section~\ref{sec:exp_efficiency}.

%\red{where is the response to the concern on the parallel training strategy? 1. respond here, and 2. update descriptions/discussions/results in the paper}


% We believe these updates and clarifications will provide a more comprehensive understanding of the OUS mechanism and its efficiency while addressing your concerns.

\vspace{2mm}
\noindent
\textbf{D1:} (4) The authors should formally define the online anomaly detection and concept drift problem. Are the definitions of concept the same for different dataset settings (continuous setting like time series data and discrete setting)? 
In time series data, it seems to be hard to learn the distribution of isolated instance without considering the temporal dependencies. How can METER handle the temporal dependencies in these time series datasets such as NYC and CPU?

\vspace{2mm}
\noindent
\textbf{Response.}% We thank you for this insightful suggestion. 
We have added formal definitions of the online anomaly detection and concept drift problem in Section~\ref{sec:preliminary} as suggested.
Notably, the concept in the context of concept drift refers to the underlying joint probability distribution $P\left( \vec{x}, y \right)$, which typically experiences only slight shifts from central concepts.
The definitions are general and applicable to different dataset settings, e.g., both continuous data with temporal dependencies like time series and discrete data without explicit temporal connections between data points.

Particularly, in the context of time series data, \name can effectively handle temporal dependencies, which consistently achieve top performance as shown in Table~\ref{tab:overall_resutls_un_con}.
To handle the temporal dependencies in datasets like NYC and CPU, we adopt the shingling approach following the convention~\cite{gopalan2019pidforest}.
With a window width of ten, this preprocessing approach transforms each data point into a 10-dimensional vector containing ten consecutive measurements.
The preprocessed vectors are then input to \name, enabling the model to capture short-term temporal dependencies within the time window.
Further, the hypernetwork-based DSD is designed to learn and capture long-term variations in the time series by dynamically generating the parameter shifts of SCD weights.
Together, they enable \name to handle the temporal dependencies in time series datasets and achieve overall the best prediction performance across different dataset settings.\\

% Such adaptive mechanism empowers \name to discern and respond to protracted shifts in data patterns effectively.

% This technique allows METER to process the newly-formed vectors and effectively capture short-term temporal dependencies within the time series window. Moreover, the advanced, hypernetwork-based DSD can adjust to the long-term variances within the time series. It learns the subtle changes in SCD weights, allowing METER to effectively recognize and adapt to prolonged alterations in the data patterns.


\vspace{2mm}
\noindent
\textbf{D2:} The effectiveness of the METER seems to be incremental. According to the ablation experiments, it seems that a well-trained vanilla autoencoder (METER-S which only uses the static concept-aware detector) can beat most baselines including incremental models and ensemble models on the INSECTS dataset (Table 4 and Table 6).

\vspace{2mm}
\noindent
\textbf{Response.} %We thank you for pointing out this issue.
To highlight the effectiveness of \name and that all the main modules, namely SCD, IEC and DSD, are indispensable for the overall best performance across datasets and settings, we have conducted a more in-depth analysis of the results in Table~\ref{tab:overall_resutls_kn_con} and Table~\ref{tab:ablation} and enhanced our discussions in Section~\ref{sec:exp_effectiveness}.

Specifically, Table~\ref{tab:overall_resutls_kn_con} shows that about half of the methods perform noticeably worse on real-world datasets with known concept drift.
Notably, although methods like MemStream obtain competitive performance on INSECT-Abr and INSECT-IncRec, they perform worse on the other two datasets, whose performance is even worse than \name using only the static concept-aware detector as shown in Table~\ref{tab:ablation}.
This phenomenon demonstrates the complexity and challenge of handling real-world OAD scenarios that are characterized by very distinct concept drifts.
% complexity of OAD when dealing with real-world datasets characterized by distinct concept drifts.
Different kinds of concept drifts require very different modeling strategies, and thus resilient models that can adapt to a wide spectrum of concept drift scenarios are much needed.
In this context, \name is effective in handling concept drift and supporting OAD, which consistently outperforms baseline models across various settings and types of concept drift, achieving overall the highest rank across datasets.

\vspace{2mm}
\noindent
\textbf{D3:}  In Fig.4, for the INSECTS-Inc dataset, the concept uncertainty at time step around 7000 is much higher than the uncertainty at time step 20000, even if an increasing trend is observed (concept shift occurring) at time step 20000. Such phenomenon needs to be discussed.

\vspace{2mm}
\noindent
\textbf{Response.} 
%We thank you for pointing out this issue for our further clarification.
We note that the concept uncertainty measures the extent to which the change of concepts in the current data stream is unexpected to the model, as detected by our intelligence evolution controller (IEC).
Hence, this phenomenon is mainly due to an initial, unexpected drift of concepts, which leads to a sudden significant increase in concept uncertainty by IEC.

Particularly, the initial drift results in a sharp spike in the concept uncertainty at the beginning of concept drift, e.g., the time step around 7000 for the INSECTS-Inc dataset, and more moderated concept uncertainty during the subsequent concept drifts, even if an increasing trend is observed, such as the concept shift occurring at time step 20000.
This phenomenon is also consistent with what we observed in INSECTS-IncGrd and INSECTS-IncRec (the last two subfigures of Fig~\ref{fig:concept_drift}).
We have enhanced the discussion of such phenomenon in Section~\ref{sec:exp_concept_drift} for clarity.\\

% We attribute this phenomenon to the initial onset of concept drift, as illustrated in the last three figures of Figure~\ref{fig:concept_drift}. In these cases, the magnitude of uncertainty undergoes a more significant shift during the initial occurrence of concept drift.
% And for the first figure, the marginally elevated uncertainty during the second instance is plausibly attributed to the pronounced occurrence of second concept drift.
% We have discussed the phenomenon in Section~\ref{sec:exp_concept_drift}. 


\vspace{2mm}
\noindent
\textbf{D4:} The interpretability of the model totally relies on the using of the evidential deep learning approach. And the efficiency of the model including both the training and inferring efficiency needs to be further validated.

\vspace{2mm}
\noindent
\textbf{Response.}% We thank you for your insightful comments and constructive suggestions.
The interpretability of the model indeed totally relies on the intelligent evolution controller (IEC), a concept detection controller that dynamically models concept uncertainty using evidential deep learning.

To validate the efficiency of the model, we have added Section~\ref{sec:exp_efficiency} that evaluates both the training and inference efficiency of \name by measuring its throughput on benchmark datasets of varying sizes and dimensions.
The results in in Table \ref{tab:efficiency} show that \name is efficient in training, and achieves very high inference efficiency, which enables rapid response for the online detection of anomalies.
Further, Table \ref{tab:efficiency} also reports the average training time for one epoch and the maximum memory usage (peak memory).
These additional results demonstrate that \name requires negligible training time and takes low memory usage across these datasets.
This is mainly due to the lightweight design of the key modules of \name, as discussed in detail in Section~\ref{sec:analysis_and_discussion}.\\

% Thanks to the reviewer for your insightful comment. The authors have carefully considered the reviewer’s suggestion and added Section~\ref{sec:exp_efficiency} to discuss the efficiency of \name including both the training and inference processes. Specifically, We evaluated the training and inference efficiency of \name by quantifying its throughput on benchmark datasets of varying sizes and dimensions. The results in Table \ref{tab:efficiency} reveal that \name is rather efficient in both training and inference phases on datasets of various sizes and dimensions. This indicates that \name exhibits high computational efficiency and possesses strong parallel computing capabilities on GPU, thus ensuring rapid response rates for real-time applications. 
% Furthermore, we also reported the average training time for each epoch and the maximum GPU memory usage (peak GPU memory) in Table \ref{tab:efficiency}. The observed trend indicates that \name exhibits relatively short training times and maintains low GPU memory usage across all datasets, which is attributed to the meticulously crafted model structure of \name, as elaborated in the discussion in Section~\ref{sec:analysis_and_discussion}.


\vspace{2mm}
\noindent
\textbf{D5:} Please clarify whether the following work can be used to solve the concept shift detection problem studied in this paper:\\
$[1]$ Bifet, A., \& Gavalda, R. (2007, April). Learning from time-changing data with adaptive windowing. In Proceedings of the 2007 SIAM international conference on data mining (pp. 443-448).\\
$[2]$ Cavalcante, R. C., Minku, L. L., \& Oliveira, A. L. (2016, July). Fedd: Feature extraction for explicit concept drift detection in time series. In 2016 International Joint Conference on Neural Networks (IJCNN) (pp. 740-747).\\
$[3]$ Huang, D. T. J., Koh, Y. S., Dobbie, G., \& Pears, R. (2014, December). Detecting volatility shift in data streams. In 2014 IEEE International Conference on Data Mining (pp. 863-868).

\vspace{2mm}
\noindent
\textbf{Response.}% We thank you for bringing these related works to our attention.
Based on the suggestion, we have taken the opportunity to expand and improve the Related Work section, highlighting the key differences between the concept drift detection approach used in these works and our targeted online anomaly detection (OAD) scenario.

Although the problem of concept drift is integral to OAD, supporting efficient and effective OAD requires more than just detecting and handling concept drift.
Further, these related works [1][2][3]
% ~\cite{bifet2007learning,cavalcante2016fedd,huang2014detecting}
focus on detecting changes in individual features or certain statistical characteristics of the data stream, e.g., mean values, within a sliding window.
However, these approaches prove to be ineffective for OAD, as concept drift in OAD exhibits more intricate changes in data distribution, such as shifts, correlations, and transformations of data patterns, which are more complex than simple statistical features used for detection as in these approaches.
Therefore, a more advanced approach, i.e., an intelligent evolution controller (IEC) that dynamically models complex concept uncertainty via evidential deep learning, is required and introduced in our \name for efficient, effective and more interpretable OAD.

% However, the approaches prove insufficient for OAD, since concept drift within OAD can encompass more intricate changes in data distribution, including shifts, correlations, and transformations of data patterns, extending beyond the scope of basic statistical features like mean values. To this end, these conventional methods fall short in addressing the complexity of OAD, where a more nuanced approach is required.

% We have enhanced and reorganized the Related Work section to include a thorough discussion of the distinctions between concept shift detection and online anomaly detection (OAD). 
% Concretely, the concept drift emerges as a critical concern in the context of online anomaly detection tasks. 
% The recommended works [1][2][3] %\cite{bifet2007learning,cavalcante2016fedd,huang2014detecting}
% relying on sliding windows primarily focus on detecting alterations in specific statistical characteristics (e.g., mean values) of streaming data or its individual features to identify concept drift. However, the approaches prove insufficient for OAD, since concept drift within OAD can encompass more intricate changes in data distribution, including shifts, correlations, and transformations of data patterns, extending beyond the scope of basic statistical features like mean values. To this end, these conventional methods fall short in addressing the complexity of OAD, where a more nuanced approach is required.\\


\vspace{2mm}
\noindent
\textbf{D6:} Some typos.\\
Fig.1 (b), the title of the second row should be “Ensemble Models”\\
P3, “interoperability” should be “interpretability”\\
P5, “the original hypernetwork…, which lack the …”\\
P6, equation 11, $\Delta t$ and $\delta t$ are not in consistent.

\vspace{2mm}
\noindent
\textbf{Response.} 
%We thank you for pointing out these typos.
We have corrected the typos and proofread the entire manuscript to ensure correctness and consistency.

% identify and rectify any potential inaccuracies.

% Thanks for pointing out these typos. We have corrected them and proofread the manuscript to ensure the elimination of typos and unclear statements.


\subsection*{Response to Reviewer 4}
\textbf{D1:} \red{a. It is not clear how the proposed framework can be adopted within a stream processing engine or CEP. For example, can it developed as a set of operators with window semantics?}

\vspace{2mm}
\noindent
\textbf{Response.} \blue{\
% We thank you for the insightful inquiry.
The online anomaly detection framework \name can be integrated with stream processing engines as a module within such engines. 
%This module is crafted to accept real-time data streams and subsequently apply online anomaly detection using the capabilities provided by \name. We have enhanced the discussions on these integration possibilities in Section~\ref{sec:analysis_and_discussion}.
%To enhance compatibility with such systems, particularly for time series data, we employ sliding window operations on streaming data, as described in Section~\ref{sec:exp_effectiveness}. As new data continually enters the system, the window dynamically shifts forward. Users can perform anomaly detection operations within the window and determine the presence of anomalies based on the data within the window. 
%In essence, although our framework does not encompass the full functionality of a stream processing engine or CEP system, it can be effectively integrated into these systems to handle online anomaly detection tasks.}
In support of this, we have introduced Section~\ref{sec:flink} to provide substantiation.
Specifically, we have integrated \name with Apache Flink, a framework and distributed processing engine for stateful computations over unbounded and bounded data streams. 
%Flink wraps \name inside a Flink operator, where Flink can help establish the required environment, manage the resource, read/write the data with the versatile connectors, and handle the failures. 
Building streaming workloads upon Flink empowers \name with real-time data processing pipelines, large-scale exploratory data analysis, and ETL processes. 
The timely output results, as depicted in Figure~\ref{fig:flink}, validate the seamless integration of \name with the streaming processing engine, reaffirming its efficacy in real-time anomaly detection.
}

%%jq: trying to test the performance of \name on flink

\vspace{2mm}
\noindent
\textbf{D1:} b. What is the memory and CPU overheads of applying the IEC and hybernetwork to a real-time application?

\vspace{2mm}
\noindent
\textbf{Response.}%Thank you for your constructive suggestion.
We have added more efficiency evaluation in the revised manuscript as a response to the question.
In Section~\ref{sec:exp_efficiency}, we evaluate the efficiency of \name in terms of both training and inference, measuring several key metrics, namely training and inference throughput, the average training time per epoch, and peak memory usage.
Results are reported in Table \ref{tab:efficiency}, which confirm that
training and inference of \name are highly efficient.

As for the memory and CPU overheads of applying the IEC and hypernetwork, we have conducted additional experiments to evaluate the efficiency of these two modules in a real-time application in Section~\ref{sec:exp_efficiency}.
Specifically, we compare peak memory usage and average training time per epoch on CPU of \name with and without IEC and hypernetwork (namely DSD).
% various variants of \name, as detailed in the ablation studies in Section~\ref{sec:exp_ablation}, including \name-S, \name-S+D, and \name without OUS.
Results show that the introduction of the IEC and DSD modules incurs a negligible increase in training time (0.014s and 0.007s, respectively) and peak memory usage (5.17MB and 2.61MB, respectively). 
Further, our ablation studies in Table \ref{tab:ablation} demonstrate that integrating these two modules into \name enhances the performance by a large margin.
These findings corroborate the efficiency and effectiveness of the IEC and hypernetwork in our framework, which is well-suited for real-time applications and supports high-performance OAD with high efficiency.\\


% Specifically, we conducted additional tests to assess the efficiency impact of the IEC and DSD modules. Specifically, we compared the average training time per epoch on CPU and peak memory usage of various variants, as detailed in Section~\ref{sec:exp_ablation}, including \name-S, \name-S+D, and \name without OUS.
% The results of these tests indicate that the inclusion of the DSD and IEC modules results in only a marginal increase in training time (0.014s and 0.007s) and peak memory usage (5.17MB and 2.61MB, respectively). 
% Considering these results alongside those presented in Table \ref{tab:ablation}, it is evident that the introduction of the DSD and IEC modules significantly enhances the model's performance while maintaining a reasonable level of overall efficiency.
% In conclusion, our efficiency experiments demonstrate that \name is well-suited for real-time applications, offering strong performance without imposing substantial memory and computational overheads.\\


\vspace{2mm}
\noindent
\textbf{D2:} a. It is not clear what kind of hardware has been used to report the performance numbers.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for pointing out this issue.
We have provided more implementation details in Section~\ref{sec:implementation_details} to include a detailed description of the hardware setting used in the experiments.
Specifically, all the experiments are conducted in a server with Xeon(R) Silver 4114 CPU @ 2.2GHz (10 cores), 256G memory, and GeForce RTX 2080 Ti.
\\


\vspace{2mm}
\noindent
\textbf{D2:} b. It is not clear how the implementation of Meter is realized. Is it deployed as an independent package of the sci-kit-learn library or integrated within an existing streaming system?

\vspace{2mm}
\noindent
\textbf{Response.} 
The key modules of \name, namely the static concept-aware detector (SCD), the intelligent evolution control (IEC), the dynamic shift-aware detector (DSD), and the offline updating strategy (OUS) are all implemented in PyTorch 1.10.0 with CUDA 10.2.
We have clarified the implementation details in Section~\ref{sec:implementation_details}.

We note that the implementation of these modules and the OAD framework can be readily integrated into existing streaming systems by sending the incoming data stream to the pipeline of \name, which can efficiently and effectively support real-time anomaly detection with better interpretability. \\

\vspace{2mm}
\noindent
\textbf{D2:} c. It is not clear how the experiment are executed. For example, did you create a data generator to emulate a streaming environment of the data sets?

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for your valuable feedback. \
We indeed created a data generator to emulate a streaming environment, and we have updated Section~\ref{sec:implementation_details} to clearly describe how the experiments are executed.

Specifically, we created a data generator that emulates the streaming data of different settings and applications.
This generator enables the systematic and controlled evaluation of \name's performance and ability to adapt to evolving data patterns and concept drift in a streaming environment.\\

% We thank you for your valuable feedback. As per your suggestion, we have incorporated a detailed explanation in Section~\ref{sec:implementation_details} regarding the data generation process. Specifically, we have created a data generator that emulates the iterative nature of streaming data. This generator facilitates the systematic and controlled assessment of \name's performance in a streaming environment, allowing us to evaluate its ability to adapt to evolving data patterns and concept drift.\\


\vspace{2mm}
\noindent
\textbf{D3:} a. The readers can benefit from a little more coverage of ML-based online anamoly detection categories including incremental learning and ensemble-based approaches, in contrast to anamoly detection.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for this valuable suggestion. W
Based on the suggestion, we have reorganized and enhanced the Related work Section~\ref{sec:related work} to provide a more comprehensive overview of the relevant research in the field of online anomaly detection.
This includes various ML-based online anomaly detection categories, particularly, incremental learning and ensemble-based approaches.
We also discuss these approaches in the context of concept drift detection, which is critical to online anomaly detection.
By enhancing this section, we aim to provide readers with a thorough understanding of the landscape of ML-based and DL-based approaches for OAD.\\


\vspace{2mm}
\noindent
\textbf{Note:} 
I guess on Figure 1 b, "Ensemble Models" on the second vertical black label instead of "Incremental Models".

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for pointing out this typo. 
We have corrected the typo in Figure~\ref{fig:intro}, where "Incremental Models" has been updated with "Ensemble Models" in the second vertical black label.
We have also thoroughly proofread the entire manuscript to ensure consistency and enhance the overall readability of the manuscript.


\subsection*{Response to Reviewer 5}
\textbf{W4:} The evaluation is not comprehensive. Experimental results cannot statistically or significantly outperform existing methods. The author address that METER is observed with consistency, but as the dataset used is not challenging enough, the take-aways are doubtful. This part would be highly improved if the author can try to apply METER on more challenging anomaly detection datasets[1]. If there is a reason why these datasets cannot be altered and used, please also give a discussion.

\vspace{2mm}
\noindent
\textbf{D3:} Evaluations seem to be extensive but requires further refinement. The proposed METER framework is compared with all competitors under different settings. Also, ablation study is conducted to show the effectiveness of each component. However, experimental results cannot statistically or significantly outperform existing methods. The author address that METER is observed with consistency, but as the dataset used is not challenging enough, the take-aways are doubtful. This part would be highly improved if the author can try to apply METER on more challenging anomaly detection datasets[1]. If there is a reason why these datasets cannot be altered and used, please also give a discussion.

\vspace{2mm}
\noindent
\textbf{R1:} Testing METER on more challenging anomaly detection datasets[1]. If there is a reason why these datasets cannot be altered and used, please also give a discussion.\\
$[1]$ https://compete.hexagon-ml.com/practice/competition/39/

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for your valuable suggestion.
We have enhanced our experimental study by adding
%this more challenging 
%anomaly detection dataset 
HexagonML (UCR) dataset as suggested.
Specifically, we adopt datasets from natural sources, namely EPG and ECG, which are the main parts of the UCR collection.
We have updated Table~\ref{tab:dataset_stats} and Section~\ref{sec:dataset} with the details of these two datasets accordingly.

Results on the two new datasets are reported in Table~\ref{tab:overall_resutls_un_con}, which further confirm that \name achieves very competitive and consistent performance across different datasets.
Notably, \name obtains the highest AUCROC of 0.968 and the second-highest AUCROC of 0.778 (very close to the best AUCROC of 0.780 achieved by MemStream on ECG) on the more challenging dataset EPG and ECG, respectively.
In contrast, although other approaches may achieve high performance on certain datasets, their performance is not consistent, and many of them fluctuate drastically across datasets.
For instance, ARCUS achieves the highest AUCPR on EPG, while it only obtains an AUCPR of 0.340, i.e., 34.99\% worse than STORM with the highest AUCPR of 0.523.\\
% We sincerely appreciate the reviewer's valuable suggestion. To address this, we have extended our experiments by incorporating the challenging anomaly detection dataset HexagonML (UCR) into our study, as elaborated in Section~\ref{sec:dataset}. 
% We selectively integrated datasets obtained from natural sources, specifically EPG and ECG, which are part of the UCR collection. Detailed statistical information about these datasets is thoughtfully presented in Table~\ref{tab:dataset_stats}.
% The results of our experiments on these datasets are documented in Table~\ref{tab:overall_resutls_kn_con}. It is noteworthy that \name has demonstrated competitive results on the UCR dataset and maintains the highest average rank within this continuous setting. 
% More details about experimental results on UCR can be found in Section~\ref{sec:exp_effectiveness}. 
% We acknowledge the importance of testing on challenging datasets, and our inclusion of HexagonML (UCR) and other datasets reflects our commitment to enhancing the robustness and comprehensiveness of our evaluation.\\

%W1 and D5 are totally the same
\vspace{2mm}
\noindent
\textbf{W1\&D5:} The contribution of this paper requires further summarization and careful refinement. The author introduces different components but fail to convey the novelty of these design. For example, hypernetwork is a typical fine-tuning method. So how does this component differentiate from incremental methods? Why not view the design of this part as an example of incremental training with fine-tuning?

\vspace{2mm}
\noindent
\textbf{D4:} Despite METER framework introduces a new paradigm, the technical depth is questionable. As mentioned in W1, why choosing these modules to form the design of METER?

%\vspace{2mm}
%\noindent
%\textbf{D5:} The contribution of this paper requires further summarization and careful refinement. The author introduces different components but fail to convey the novelty of these design. For example, hypernetwork is a typical fine-tuning method. So how does this component differentiate from incremental methods? Why can’t we view the design of this part as an example of incremental training with fine-tuning?

\vspace{2mm}
\noindent
\textbf{R2:} Discuss more about the novelty and contribution of the design of hypernetwork. Answer the below questions. (1) How does this component differentiate from incremental methods? (2) Why can’t we view the design of this part as an example of incremental training with fine-tuning? This part can be further discussed, and if there is already some discussion, please highlight them.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for pointing out the novelty issue.
As a response, we have 
%taken %this opportunity 
%to clarify and further highlight
clarified 
the novelty and 
contributions of the paper, and also illustrated the technical depth of our \name more clearly.

We clarify that our hypernetwork-based approach is a new paradigm that is very different from existing incremental approaches or ensemble approaches.
Particularly, as compared with incremental approaches, (1) in deployment, namely after the model training, the hypernetwork can dynamically generate the \textit{parameter shift} for the current data stream to handle the concept drifts on the fly and enhance the predictive performance of the base detection model without further fine-tuning or training, whereas incremental approaches need to update their detection models to accommodate the changing concepts, typically by retraining, fine-tuning, or updating certain model statuses when concept drift is detected in the data stream~\cite{bhatia2022memstream,yoon2021multiple,yoon2020ultrafast}. Therefore, our hypernetwork approach can instantly adapt to changing concepts, and thus is more \textit{efficient} and \textit{effective} in handling concept drift for OAD than incremental approaches.
(2) To further improve \textit{efficiency} for real-time OAD and \textit{interpretability} for informed decision-making and critical applications, we design \textit{dynamic concept adaptation} with the two novel modules, the intelligent evolution controller (IEC) and the dynamic shift-aware detector (DSD, i.e., the hypernetwork), where the hypernetwork is only invoked to handle the changing concepts when necessary.
Specifically, a lightweight and evidential deep learning theory-based controller is introduced to model the concept uncertainty and decide whether the hypernetwork is required to handle the changing concepts \textit{in an input-aware manner}.
In contrast, existing incremental approaches lack support for interpretability and are not able to support such a fine-grained solution for addressing concept drift in OAD.

\blue{We have improved the Introduction section, Section~\ref{sec:analysis_and_discussion}, and Related Work to highlight the differences and novelties of our \name compared with existing approaches.}
% sf: add these discussions to the paper.


\vspace{2mm}
\noindent
\textbf{W2\&D6:} The motivation of METER design is unclear. How can these techniques solve the challenge OAD faces? In Section I, the author claim METER is built upon the observation that ‘static historical data typically encompass the majority of anomaly patterns and thus comprises the recurring central concepts’. More experiments are required to demonstrate this observation. This discovery could be the highlight of this work, which can motivate more exploration in this direction.

%\vspace{2mm}
%\noindent
%\textbf{D6:} The motivation of METER design is unclear. How can these techniques solve the challenge OAD faces? In Section I, the author claim METER is built upon the observation that ‘static historical data typically encompass the majority of anomaly patterns and thus comprises the recurring central concepts’. More experiments are required to demonstrate this observation. This discovery could be the highlight of this work, which can motivate more exploration in this direction.

\vspace{2mm}
\noindent
\textbf{R3:} Provide more experimental results to prove the observation that ‘static historical data typically encompass the majority of anomaly patterns and thus comprises the recurring central concepts’.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for your valuable feedback and constructive suggestions.
\blue{We have clarified the motivation of \name design and explained how these techniques solve the main challenge of concept drift in OAD in the Introduction section, Section~\ref{sec:analysis_and_discussion}, and Related Work.
Please refer to our response to W1\&D2, D4, and R2 above for details and discussions.}

In addition, we have added ablation studies to demonstrate the key observation that 'static historical data typically encompass the majority of anomaly patterns and thus comprises the recurring central concepts' in Section~\ref{sec:exp_ablation}.
Specifically, we partition the INSECTS-Abr dataset into five sequential and equal subsets, denoted as $p_1$ to $p_5$.
Then, we further split each subset into one training set and one test set, and derive $p_{1-train}/p_{1-test}$ to $p_{5-train}/p_{5-test}$ correspondingly.
Using these subsets, we conduct two groups of experiments.
In Group I, we train \name on $p_{1-train}$ and then fine-tune \name on $p_{2-train}$ to $p_{5-train}$ respectively, and report the detection performance of \name.
Such an initial training and subsequent fine-tuning strategy is widely adopted in conventional incremental and ensemble approaches.
As for the experiments of Group II, we only train \name on $p_{1-train}$ once, and then report the trained \name on all test sets, namely $p_{1-test}$ to $p_{5-test}$.

Results summarized in Table~\ref{tab:reccurring} show that (1) the fine-tuning strategy is not effective in OAD, which may lead to worse performance than the model initially trained but without fine-tuning, e.g., the Group I model archives an AUCROC of 0.702 on $p_{4-test}$, which is much worse than 0.754 of the Group II model without further fine-tuning.
(2) The model of Group II archives an AUCROC of 0.768, which is only slightly worse than 0.804 obtained on $p_{1-test}$, and obtains an even higher AUCROC of 0.837 on $p_{5-test}$.
These two findings suggest that the majority of anomaly patterns are indeed already encompassed on the status historical data, namely $p_{1-train}$, and the model of Group II only trained on $p_{1-train}$ can, to a large extent, detect most anomalies on the subsequent unseen test sets, which achieve so by learning the recurring central concepts encompassed in the static historical data.
We have also conducted experiments on other datasets, such as BGL, NYC, and SynM-GrdRec, and observed consistent results.
These empirical results confirm this observation.
We have provided discussions and in-depth analysis in Section~\ref{sec:exp_ablation} to demonstrate and explain this observation.
\\

% In response to the reviewer's suggestion, we have expanded our ablation study to provide additional experimental evidence supporting the observation that static historical data generally contains the majority of anomaly patterns.
% To achieve this, we divided the INSECTS-Abr dataset into 5 equal parts, denoted as $p_1-p_5$. Within each part, we further divided the data into training and test sets using a 0.2/0.8 ratio, resulting in $p_{1tr}-p_{5tr}$ and $p_{1te}-p_{5te}$, respectively. We conducted two sets of comparative experiments. In the first set, we initially trained \name on $p_{1tr}$ and then fine-tuned it on $p_{2tr}-p_{5tr}$ individually. In the second set, \name was exclusively trained on $p_{1tr}$. The results of inference on $p_{1te}-p_{5te}$ are presented in Table~\ref{tab:reccurring}.
% From the results, it is evident that the mean values of the two groups exhibit slight differences, aligning with the notion that static historical data typically encompasses the majority of anomaly patterns. Furthermore, the superior and less variable outcomes in group II provide additional validation of the effectiveness of the Offline Updating Strategy (OUS) in handling recurring central concepts. For a more detailed analysis, please refer to Section~\ref{sec:exp_ablation} of the paper.\\


\vspace{2mm}
\noindent
\textbf{W3\&D7:} The flexibility of METER is not explored thoroughly. METER is demonstrated in this paper as a framework using IEC and DSD as key components to facilitate concept detection. The author should have tested different design of SCD module.

%\vspace{2mm}
%\noindent
%\textbf{D7:} The flexibility of METER is not explored thoroughly. METER is demonstrated in this paper as a framework using IEC and DSD as key components to facilitate concept detection. The author should have tested different design of SCD module.

\vspace{2mm}
\noindent
\textbf{R4:} The author should have tested different design of SCD module to prove the flexibility of METER.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for your valuable suggestion.
We have conducted more ablation studies to test different designs of the SCD module to prove the flexibility of \name.
Specifically, we have tested LSTM, 1D convolution, and 1D convolution with residual connections for the SCD module.
We adopt these three representative designs of the SCD module in order to demonstrate that the design of our \name framework is flexible and the base detection model, namely the SCD module, can be readily enhanced by adopting other more advanced models.

Results in Table~\ref{tab:ablation_instance-specific} show that all the three enhanced SCD modules can achieve noticeably better detection performance, with an increase in AUCROC of 7.57\%, 3.59\%, and 6.03\% respectively, as compared to the original SCD module based on a canonical DNNs.
These results further confirm the effectiveness and flexibility of our \name framework.



% Thank you for your insightful comment. We have taken your suggestion into account and expanded our ablation study to demonstrate the flexibility of \name.
% In our study, we conducted an extensive evaluation of various SCD module designs, including LSTM, 1D convolution, and 1D convolution with residual connections. These experiments were aimed at thoroughly exploring METER's adaptability and versatility in handling different SCD architectures. The comprehensive results are presented in Table~\ref{tab:ablation instance-specific}, highlighting the commendable performance of all three variants. Importantly, they outperformed the SCD module in the DNNs implementation, reaffirming METER's adaptability. Furthermore, these findings suggest promising opportunities for further enhancing METER's performance. For more detailed results, please refer to Section~\ref{sec:exp_ablation}.\\


\vspace{2mm}
\noindent
\textbf{W5\&D8:} Interpretability is introduced as a challenge but demonstrated carelessly. As this concept is still a mysterious filed and hasn’t come to a unified definition, it is preferred to use some citation to support the claim. If this cannot be a more vivid case study (with task case scenario generating the data) can also do the trick.

%\vspace{2mm}
%\noindent
%\textbf{D8:} Interpretability is introduced as a challenge but demonstrated carelessly. As this concept is still a mysterious filed and hasn’t come to a unified definition, it is preferred to use some citation to support the claim. If this cannot be a more vivid case study (with task case scenario generating the data) can also do the trick.

\vspace{2mm}
\noindent
\textbf{R5:} Add some citation or similar work to support this understanding of interpretability in this paper. If this cannot be satisfied, a more vivid case study (with task case scenario generating the data) can also do the trick.

\vspace{2mm}
\noindent
\textbf{Response.}%We thank you for your valuable feedback and constructive suggestions.
We have enhanced the analysis and discussions on interpretability in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability}.
As suggested, we have added additional citations and similar works to aid the understanding of interpretability in our paper.
%These citations and new discussions indeed facilitate the understanding and improve the clarity of interpretability of our OAD framework.
\\


% Thanks for your thoughtful and detailed comment. Following your suggestion, we have conducted a more detailed analysis in Section~\ref{sec:analysis_and_discussion} and Section~\ref{sec:exp_interpretability}.
% Furthermore, we have incorporated relevant citations that align with our discussions on interpretability in Section~\ref{sec:analysis_and_discussion}. 
% These revisions aim to strengthen the comprehension of interpretability in our paper, as well as provide supporting evidence from existing research in the field.\\


%Finally, we extend our sincere appreciation to the reviewers for their insightful and constructive comments, which have significantly enhanced the quality of our research and the paper. The valuable feedback we've received has contributed to making this manuscript more comprehensible and persuasive compared to the earlier version. We trust that these revisions provide a stronger contribution to the field.

\end{multicols}



\setcounter{page}{5}

==> secs/8.acknowledgement.tex <==
\section{ACKNOWLEDGMENTS}\label{sec:acknowledgement}

This work is supported by the National Research Foundation, Singapore under its Emerging Areas Research Projects (EARP) Funding Initiative. 
Any opinions, findings and conclusions or recommendations expressed in this material are those of the author(s) and do not reflect the views of National Research Foundation, Singapore. 
The work is also supported by the National Natural Science Foundation of China National Science Fund for Distinguished Young Scholars 62025301, 
and the National Natural Science Foundation of China under Grant 61933002.
